RDMA Performance Isolation With Justitia

Despite its increasing popularity, most of RDMA's benefits such as ultra-low latency can be achieved only when running an application in isolation. Using microbenchmarks and real open-source RDMA applications, we identify a series of performance anomalies when multiple applications coexist and show that such anomalies are pervasive across InfiniBand, RoCEv2, and iWARP. They arise due to a fundamental tradeoff between performance isolation and work conservation, which the state-of-the-art RDMA congestion control protocols such as DCQCN cannot resolve. We present Justitia to address these performance anomalies. Justitia is a software-only, host-based, and easy-to-deploy solution that maximizes RNIC utilization while guaranteeing performance isolation via shaping, rate limiting, and pacing at senders. Our evaluation of Justitia on multiple RDMA implementations show that Justitia effectively isolates different types of traffic and significantly improves latency (by up to 56.9x) and throughput (by up to 9.7x) of real-world RDMA-based applications without compromising low CPU usage or modifying the applications.

==> ack.tex <==
\section*{Acknowledgments}


==> background.tex <==
%!TEX root=frdma.tex
\section{RDMA Primer}
\label{sec:background}
In this section, we provide a quick overview of RDMA, existing RDMA implementations, and RDMA NICs.

\begin{table}[!t]
  \caption{RDMA Transport Types and Communication Verbs.}
  \label{tab:transport-verbs}
  \small
  \begin{tabular}{cccccc}
    \toprule
    & SEND & RECEIVE & WRITE/WIMM & READ\\
    \midrule
   \bf{RC} & \checkmark & \checkmark & \checkmark & \checkmark \\ 
   \bf{UC} & \checkmark & \checkmark & \checkmark & \\ 
   \bf{UD} & \checkmark & \checkmark &  & \\ 
   \bottomrule
  \end{tabular}
\end{table}

\subsection{Fundamentals of RDMA}
RDMA allows direct access to the remote machine's memory without involving the CPU or operating system of either host. 
It has three primary implementations (\S\ref{sec:rdma-impl}), all of which are rooted in the Virtual Interface Architecture (VIA) abstract model \cite{via-1, via-2}. 
VIA is based on two synergistic concepts: \emph{applications have direct access to a network interface} and \emph{applications directly exchange in-memory data across the network}, all bypassing the operating system.

\paragraph{RDMA Verbs}
RDMA NICs expose the \emph{verbs} API to applications for directly accessing the network interface using queue pairs (QP).
Each QP consists of a send queue and a receive queue. 
To perform an operation, a work queue element (WQE) is placed in the appropriate work (send or receive) queue.
Upon completion of an operation, a completion queue element (CQE) is inserted at the tail of the completion queue (CQ) associated with the QP.

RDMA verbs use one of the two transfer semantics; \eg, SEND and RECEIVE follow the channel semantic like TCP/IP, while READ and  WRITE use the memory semantic.

\paragraph{Transport Types}
Current RDMA implementations support three transport types: Reliable Connection (RC), Unreliable Connection (UC), and Unreliable Datagram (UD).
RC supports guaranteed-order packet delivery by enforcing packet acknowledgement.
Connected transports (RC, UC) require one-to-one QP, while single QP can communicate with multiple QPs in connectionless transport (UD).
% Therefore, UD can offer better scalability to some applications \cite{herd, rdma-design-guideline, fasst-osdi16}.
However, not all transport types support all communication verbs (Table~\ref{tab:transport-verbs}). 
% The RDMA standard also provides two atomic operations for implementing distributed shared memory \cite{rfc7306}.


\subsection{RDMA Implementations}
\label{sec:rdma-impl}
\paragraph{InfiniBand}
% InfiniBand is a switch-based serial I/O interconnect architecture \cite{ib-intro}.
% It operates both on the PCB as a component-to-component interconnect as well as an ``out of the box'' chassis-to-chassis interconnect.
InfiniBand provides an application with a rich set of I/O services based on the RDMA access methods and message passing semantics in an InfiniBand-defined network.
In the link layer, InfiniBand applies a credit-based approach for lossless flow control \cite{ib-arch-spec-1}.
It also supports QoS via a limited number of virtual lanes (typically, 15) \cite{ib-arch-spec-1}.

\paragraph{RoCE}
RDMA over Converged Ethernet (RoCE) is a standard protocol to provide InfiniBand transport services on Ethernet networks.
It preserves the InfiniBand verbs semantics together with its transport and network protocols, and it replaces the InfiniBand link and physical layers with Ethernet \cite{ibta-roce-v2}.
While RoCE provides communication within an Ethernet L2 domain, RoCEv2 extends the RoCE protocol to allow packets to be routed across Ethernet boundaries \cite{msr-rdma-15, msr-rdma-16}.

\paragraph{iWARP}
Internet Wide-area RDMA Protocol (iWARP) delivers converged, low-latency fabric services by supporting transmission over TCP and is implemented on top of IP networks using an existing Ethernet infrastructure.
Besides including the kernel-bypass and zero-copy feature of RDMA, iWARP accelerates transport processing by utilizing the network controller instead of the processor \cite{understand-iWARP}.

% \subsubsection{LITE}
% LITE \cite{lite} is a recent software-based RDMA implementation that adds a local indirection layer for RDMA in the Linux kernel to virtualize native RDMA into a flexible high-level abstraction.
% It onloads privileged resources management into the kernel, but it still preserves RDMA's low-latency performance benefits while avoiding drawbacks caused by RDMA's kernel bypassing.
% LITE also removes scalability bottlenecks of the RNIC hardware.

\subsection{Multi-Resource RDMA NICs}
Despite the differences, RDMA NICs for all three architectures share some commonalities.
In particular, in all of them, two primary resources need to be shared amongst competing QPs on an RNIC: \emph{link bandwidth} and \emph{execution unit throughput}. 
First, bandwidth is limited on any RNIC, and the NIC must share its bandwidth between different QPs by deciding when to send packets from each QP. 
Also, because RDMA NICs offload messaging and packetization to the NIC, RDMA NICs also have execution units that are responsible for reading individual verbs posted to different QPs and generating valid packets.
At small verb sizes, the number of operations per second supported by the NIC may limit throughput before bandwidth~\cite{rdma-design-guideline}.  
As a result, NIC throughput in terms of messages per second is also a resource that needs to be shared between different QPs.
% Note: DMA/memory is also a shared resource. For now this discussion
% ignores this.

